Supervised structure learning

This paper concerns structure learning or discovery of discrete generative models. It focuses on Bayesian model selection and the assimilation of training data or content, with a special emphasis on the order in which data are ingested. A key move - in the ensuing schemes - is to place priors on the selection of models, based upon expected free energy. In this setting, expected free energy reduces to a constrained mutual information, where the constraints inherit from priors over outcomes (i.e., preferred outcomes). The resulting scheme is first used to perform image classification on the MNIST dataset to illustrate the basic idea, and then tested on a more challenging problem of discovering models with dynamics, using a simple sprite-based visual disentanglement paradigm and the Tower of Hanoi (cf., blocks world) problem. In these examples, generative models are constructed autodidactically to recover (i.e., disentangle) the factorial structure of latent states - and their characteristic paths or dynamics.

==> active_learning.tex <==
\section{Active learning}\label{sec:active_learning}

Active learning has a special meaning in this paper. It implies that the act of updating Dirichlet counts is selected on the basis of expected free energy; where expected free energy—from the perspective of model parameters—is, effectively, the mutual information encoded by the tensors: see Equation \ref{eq:3}. Put simply, this means that an update is selected in proportion to the expected information gain. Consider two actions: to update or not to update. From Figure \ref{fig:figure_2}, we have (dropping the modality superscript for clarity):

\begin{equation}
\begin{aligned} & \Delta \mathbf{a}=\mathbf{o}_\tau \otimes_{i \in p a} \mathbf{s}_\tau^i \\ & \mathbb{E}[P(o, s \mid a)]=\bar{a}=: \frac{a}{\Sigma(a)} \\ & \mathbb{E}_Q\left[a \mid u=u_o\right]=\mathbf{a} \mid u_o=\mathbf{a} \\ & \mathbb{E}_Q\left[a \mid u=u_1\right]=\mathbf{a} \mid u_1=\mathbf{a}+\Delta \mathbf{a}\end{aligned}
\label{eq:5}
\end{equation}


Here, $\Sigma(a)=\mathbf{1} \odot a \odot_{i \in p a} \mathbf{1}$ is just the sum of all tensor elements. The prior probability of committing to an update is given by the expected free energy of the respective Dirichlet parameters, which scores the expected information or gain (i.e., mutual information) and cost\footnote{For simplicity, we assume tensors have been formatted as matrices, by vectorising the second and trailing dimensions.}:

\begin{equation}
\begin{aligned} P(u) & =\sigma(-\alpha \cdot G(\mathbf{a} \mid u)) \\ G(\mathbf{a}) & =-\underbrace{\mathbb{E}_{Q_a}\left[D_{K L}[P(s, o \mid \mathbf{a}) \| P(s \mid \mathbf{a}) P(o \mid \mathbf{a})]\right.}_{\text {mutual information }}-\underbrace{\mathbb{E}_{Q_a}[\ln P(o \mid c)]}_{\text {expected cost }} \\ & =(\mathbf{1} \odot \overline{\mathbf{a}}) \odot \ell(\mathbf{1} \odot \overline{\mathbf{a}})+(\overline{\mathbf{a}} \odot \mathbf{1}) \odot \ell(\overline{\mathbf{a}} \odot \mathbf{1})-\mathbf{1} \odot(\overline{\mathbf{a}} \times \ell(\overline{\mathbf{a}})) \odot \mathbf{1}-\varphi(\mathbf{c}) \odot(\overline{\mathbf{a}} \odot \mathbf{1})
\label{eq:6}
\end{aligned}
\end{equation}

This prior over the updates furnishes a Bayesian model average of the likelihood parameters, effectively marginalising over update options:

\begin{equation}
\begin{aligned} \mathbb{E}_Q\left[a_{\tau+1}^g\right] & =P\left(u_0\right) \cdot \mathbb{E}_Q\left[a_\tau^g \mid u=u_o\right]+P\left(u_1\right) \mathbb{E}_Q\left[a_\tau^g \mid u=u_i\right] \\ & \Rightarrow \\ \mathbf{a}_{\tau+1}^g & =P\left(u_0\right) \cdot \mathbf{a}_\tau^g+P\left(u_1\right)\left(\mathbf{a}_\tau^g+\Delta \mathbf{a}_\tau^g\right) \\ & =\mathbf{a}_{\tau}^g+P\left(u_1\right) \Delta \mathbf{a}_\tau^g\end{aligned}
\label{eq:7}
\end{equation}

In equation \ref{eq:6}, $\alpha$ plays the role of a hyperprior that determines the sensitivity to expected free energy. When this precision parameter is large, the Bayesian model average above becomes Bayesian model selection; i.e., either the update is selected, or it is not. 

